Joint data rate and EMF exposure analysis in Manhattan environments: stochastic geometry and ray tracing approaches

The objective of this study is to jointly analyze the data rate and electromagnetic field (EMF) exposure in urban environments. Capitalizing on stochastic geometry (SG), a network level analysis is performed by modelling these environments via Manhattan Poisson line processes (MPLP). Using this framework, a number of performance metrics are derived: first moments, marginal distributions and joint distributions of the data rate and exposure. In addition, the original Manhattan model is generalized to include advanced features: corner diffraction, presence of potential blockages in streets, and users positioned at crossroads. As a second approach, deterministic ray tracing (RT) is utilized to compute the same metrics. The two methods are shown to provide close results on the condition that the model parameters are coherently selected. Furthermore, the numerical results enable to gain insight into several aspects: the role of the propagation mechanisms in the performance metrics, existing trade-offs between the rate and exposure requirements, as well as the impact of the user location (at a crossroad or in a single street). (This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible)

==> Appendices.tex <==
  %%%%%%%
  %%%%%%%
  \section{Proof of Equation \eqref{eqcharfunL}: characteristic function for the LOS interfering links}
  \label{eqcharfunLProof}
  This proof is inspired by \cite{elsawy2016modeling}. Let $\Phi_{L}(r)$ be the set of interfering BSs located in the typical street in LOS conditions located further than a distance $r$ from the centric user. We denote by $\left|h_j\right|^2$, the fading coefficients associated to a BS $j \in \Phi_L$ and $r_j$, its distance to the typical user. The characteristic function of the interference coming from $\Phi_{L}(r)$ can be expressed as 
  \begin{align*}
    \phi_{L,1}(t|r)  &= \mathbb{E}_{\Phi_{L}(r)}\left[\prod_{j \in \Phi_{L}(r) } \mathbb{E}_{\left|h_j\right|^2}\left[\exp{\left(  jtP_B\left|h_j\right|^2\kappa_L^{-1}\sqrt{r_j^2 + \Delta H^2}^{-\alpha_L} \right) }  \right]\right] \\
    &\stackrel{(1)}{=} \exp \left(-2\lambda_{B}\int_{r}^R  p_L(r')\Bigg[1- \mathbb{E}_{\left|h\right|^2}\left[\exp{\left(  jtP_B\left|h\right|^2\kappa_L^{-1}\sqrt{r'^2 + \Delta H^2}^{-\alpha_L} \right) }  \right]\Bigg] dr' \right)   \nonumber\\
    &\stackrel{(2)}{=} \exp\Bigg[2\lambda_{B}\int_{r}^{R} p_{L}(r')\bigg[ \phi_F\Big(P_B\kappa_L^{-1}\sqrt{r'^2 +\Delta H^2}^{-\alpha_L}t;K\Big) - 1\bigg] dr' \Bigg].
   \end{align*}
   \normalsize

(1) comes is obtained by definition of the probability generating functional (PGFL) of $\Phi_L$; (2) comes from the definition of the characteristic function $\Phi_F(\cdot;\cdot)$.
  
  %%%%%%%
  \section{Proof of Equation \eqref{eqcharfunD}: characteristic function of the diffracted links}
  \label{eqcharfunDProof}
  For this proof, the following notations are introduced:
  \begin{itemize}
      \item $\Psi_{VS}$ it the 1D PPP of the intersections of the vertical streets with the typical UE avenue.
      \item $y_k$ is the distance between the typical UE and the crossroad with vertical street $k\in \Psi_{VS}$. 
      \item $\Psi_{b,k}$ it the 1D PPP of the BSs present in vertical street $k$.
      \item $x_{jk}$ is the distance from BS $j \in \Psi_{b,k}$ to the crossroad of street $k$ with the user street. 
  \end{itemize}

In the following computations, we denote $\delta = jtP_B\kappa_D^{-1}$.
\begin{align*}
    \phi_{D,1}(t|r)  &= \mathbb{E}_{\Psi_{VS}}\left[\mathbb{E}_{\Psi_{b,k}}\left[ \mathbb{E}_{\left|h_{jk}\right|^2}\left[ \exp{\left( \sum_{y_k \in \Phi_{VS}} \sum_{x_{jk} \in \Phi_{b,k}} \delta\left|h_{jk}\right|^2\mathcal{D}_b(x_{jk},y_{k})^{-\alpha_D}\right) }  \right]  \right] \right] \nonumber\\
    &= \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}} \mathbb{E}_{\Psi_{b,k}}\left[\prod_{x_{jk} \in \Psi_{b,k}} \mathbb{E}_{\left|h_{jk}\right|^2}\left[\exp{\left(  \delta\left|h_{jk}\right|^2\mathcal{D}_b(x_{jk},y_{k})^{-\alpha_D} \right) }  \right]\right] \right] \nonumber\\
    &\stackrel{(1)}{=} \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}} \mathbb{E}_{\Psi_{b,k}}\left[\prod_{x_{jk} \in \Psi_{b,k}} \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big) \right] \right] \nonumber\\
    &\stackrel{(2)}{=} \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}}  \exp \left(-2\lambda_{B}\int_{r_s}^R  1- \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big) dx \right)\right] \\ \nonumber
    &\stackrel{(3)}{=} \exp \Bigg[-2\lambda_{S}\int_{0}^R  1- \exp \Big[-2\lambda_{B}\int_{r_s}^R  1- \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big)  dx \Big]dy\Bigg]\nonumber  \nonumber
 \end{align*}
 \normalsize
(1) is obtained by computing the expectation of the fading coefficients, and by definition of $\Phi_F(\cdot,\cdot)$. (2) and (3) come from the definition of the PGFL \cite{baccelibook}, applied on $\Psi_{b,k}$ then on $\Psi_{VS}$.

  %%%%%%%
  \section{Proof of Equation \eqref{eqCovprob}: coverage probability of a typical UE}
  \label{eqCovprobProof}
  Conditioned on the serving distance $r$ and on $(p)$, the propagation condition of the serving BS (LOS or NLOS), the coverage probability can be expressed as: 
  \small
  \begin{align*}
    P_{c,q}^{(p)}(\theta_c|r)  &\stackrel{(1)}{=} \mathbb{P}\left[\left.S-\theta_c\left(I_L +I_N +I_D\right)>0\right|r\right] \nonumber\\
    &\stackrel{(2)}{=} \dfrac{1}{2} + \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{S}^{(p)}(t|r)\phi_{L,q}(-\theta_c t|r) \phi_{N,q}(-\theta_c t|r)\phi_{D,q}(-\theta_c t) \bigg] t^{-1}dt. \nonumber
   \end{align*}
    \normalsize
   (1) is obtained by definition of the coverage probability and by rearranging terms and (2) is computed using the Gil-Pelaez theorem \cite{gil1951note}. The desired expression is then obtained as follows:
   \small
   \begin{align}
    P_{c,q}(\theta_c)&\stackrel{(1)}{=} \int_{r_0}^{R}  \left(p_L(r)P_{c,q}^{(L)}(\theta_c|r) + p_N(r)P_{c,q}^{(N)}(\theta_c|r) \right)f_{r,q} (r)dt \nonumber\\  
    &\stackrel{(2)}{=} \dfrac{1}{2} + \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{D,q}(-\theta_c t) \int_{r_0}^{R}p_L(r)\phi_{S}^{(L)}(t|r)\phi_{L,q}(-\theta_c t|r)\phi_{N,q}(-\theta_c t|r)f_{r,q}(r)dr \bigg] t^{-1}dt \nonumber\\
    & ~\quad ~\quad+ \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{D,q}(-\theta_c t) \int_{r_0}^{R}p_N(r)\phi_{S}^{(N)}(t|r)\phi_{L,q}(-\theta_c t|r)\phi_{N,q}(-\theta_c t|r)f_{r,q}(r)dr \bigg] t^{-1}dt \nonumber
   \end{align}
    \normalsize
   (1) is obtained by averaging over the distibution of the serving distance and by using the total law of probability; (2) is obtained by developing the expressions of the conditioned probabilities.
  %%%%%%%%%%%%%%%%%%%%%%%%%%
  

==> Manhattan_paper_2_columns arxiv/Appendices.tex <==
  %%%%%%%
  %%%%%%%
  \section{Proof of Equation \eqref{eqcharfunL}: characteristic function for the LOS interfering links}
  \label{eqcharfunLProof}
  This proof is inspired by \cite{elsawy2016modeling}. Let $\Phi_{L}(r)$ be the set of interfering BSs located in the typical street in LOS conditions located further than a distance $r$ from the centric user. We denote by $\left|h_j\right|^2$, the fading coefficients associated to a BS $j \in \Phi_L$ and $r_j$, its distance to the typical user. The characteristic function of the interference coming from $\Phi_{L}(r)$ can be expressed as 
  \begin{align*}
    \phi_{L,1}(t|r)  &= \mathbb{E}_{\Phi_{L}(r)}\left[\prod_{j \in \Phi_{L}(r) } \mathbb{E}_{\left|h_j\right|^2}\left[\exp{\left(  jtP_B\left|h_j\right|^2\kappa_L^{-1}\sqrt{r_j^2 + \Delta H^2}^{-\alpha_L} \right) }  \right]\right] \\
    &\stackrel{(1)}{=} \exp \left(-2\lambda_{B}\int_{r}^R  p_L(r')\Bigg[1- \mathbb{E}_{\left|h\right|^2}\left[\exp{\left(  jtP_B\left|h\right|^2\kappa_L^{-1}\sqrt{r'^2 + \Delta H^2}^{-\alpha_L} \right) }  \right]\Bigg] dr' \right)   \nonumber\\
    &\stackrel{(2)}{=} \exp\Bigg[2\lambda_{B}\int_{r}^{R} p_{L}(r')\bigg[ \phi_F\Big(P_B\kappa_L^{-1}\sqrt{r'^2 +\Delta H^2}^{-\alpha_L}t;K\Big) - 1\bigg] dr' \Bigg].
   \end{align*}
   \normalsize

(1) comes is obtained by definition of the probability generating functional (PGFL) of $\Phi_L$; (2) comes from the definition of the characteristic function $\Phi_F(\cdot;\cdot)$.
  
  %%%%%%%
  \section{Proof of Equation \eqref{eqcharfunD}: characteristic function of the diffracted links}
  \label{eqcharfunDProof}
  For this proof, the following notations are introduced:
  \begin{itemize}
      \item $\Psi_{VS}$ it the 1D PPP of the intersections of the vertical streets with the typical UE avenue.
      \item $y_k$ is the distance between the typical UE and the crossroad with vertical street $k\in \Psi_{VS}$. 
      \item $\Psi_{b,k}$ it the 1D PPP of the BSs present in vertical street $k$.
      \item $x_{jk}$ is the distance from BS $j \in \Psi_{b,k}$ to the crossroad of street $k$ with the user street. 
  \end{itemize}

In the following computations, we denote $\delta = jtP_B\kappa_D^{-1}$.
\begin{align*}
    \phi_{D,1}(t|r)  &= \mathbb{E}_{\Psi_{VS}}\left[\mathbb{E}_{\Psi_{b,k}}\left[ \mathbb{E}_{\left|h_{jk}\right|^2}\left[ \exp{\left( \sum_{y_k \in \Phi_{VS}} \sum_{x_{jk} \in \Phi_{b,k}} \delta\left|h_{jk}\right|^2\mathcal{D}_b(x_{jk},y_{k})^{-\alpha_D}\right) }  \right]  \right] \right] \nonumber\\
    &= \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}} \mathbb{E}_{\Psi_{b,k}}\left[\prod_{x_{jk} \in \Psi_{b,k}} \mathbb{E}_{\left|h_{jk}\right|^2}\left[\exp{\left(  \delta\left|h_{jk}\right|^2\mathcal{D}_b(x_{jk},y_{k})^{-\alpha_D} \right) }  \right]\right] \right] \nonumber\\
    &\stackrel{(1)}{=} \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}} \mathbb{E}_{\Psi_{b,k}}\left[\prod_{x_{jk} \in \Psi_{b,k}} \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big) \right] \right] \nonumber\\
    &\stackrel{(2)}{=} \mathbb{E}_{\Phi_{VS}}\left[\prod_{y_k \in \Psi_{VS}}  \exp \left(-2\lambda_{B}\int_{r_s}^R  1- \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big) dx \right)\right] \\ \nonumber
    &\stackrel{(3)}{=} \exp \Bigg[-2\lambda_{S}\int_{0}^R  1- \exp \Big[-2\lambda_{B}\int_{r_s}^R  1- \Phi_F\Big(P_B\kappa_D^{-1}\mathcal{D}_b(x,y)^{-\alpha_D}t;0\Big)  dx \Big]dy\Bigg]\nonumber  \nonumber
 \end{align*}
 \normalsize
(1) is obtained by computing the expectation of the fading coefficients, and by definition of $\Phi_F(\cdot,\cdot)$. (2) and (3) come from the definition of the PGFL \cite{baccelibook}, applied on $\Psi_{b,k}$ then on $\Psi_{VS}$.

  %%%%%%%
  \section{Proof of Equation \eqref{eqCovprob}: coverage probability of a typical UE}
  \label{eqCovprobProof}
  Conditioned on the serving distance $r$ and on $(p)$, the propagation condition of the serving BS (LOS or NLOS), the coverage probability can be expressed as: 
  \small
  \begin{align*}
    P_{c,q}^{(p)}(\theta_c|r)  &\stackrel{(1)}{=} \mathbb{P}\left[\left.S-\theta_c\left(I_L +I_N +I_D\right)>0\right|r\right] \nonumber\\
    &\stackrel{(2)}{=} \dfrac{1}{2} + \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{S}^{(p)}(t|r)\phi_{L,q}(-\theta_c t|r) \phi_{N,q}(-\theta_c t|r)\phi_{D,q}(-\theta_c t) \bigg] t^{-1}dt. \nonumber
   \end{align*}
    \normalsize
   (1) is obtained by definition of the coverage probability and by rearranging terms and (2) is computed using the Gil-Pelaez theorem \cite{gil1951note}. The desired expression is then obtained as follows:
   \small
   \begin{align}
    P_{c,q}(\theta_c)&\stackrel{(1)}{=} \int_{r_0}^{R}  \left(p_L(r)P_{c,q}^{(L)}(\theta_c|r) + p_N(r)P_{c,q}^{(N)}(\theta_c|r) \right)f_{r,q} (r)dt \nonumber\\  
    &\stackrel{(2)}{=} \dfrac{1}{2} + \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{D,q}(-\theta_c t) \int_{r_0}^{R}p_L(r)\phi_{S}^{(L)}(t|r)\phi_{L,q}(-\theta_c t|r)\phi_{N,q}(-\theta_c t|r)f_{r,q}(r)dr \bigg] t^{-1}dt \nonumber\\
    & ~\quad ~\quad+ \dfrac{1}{\pi} \int_{0}^{\infty} Im\bigg[\phi_{D,q}(-\theta_c t) \int_{r_0}^{R}p_N(r)\phi_{S}^{(N)}(t|r)\phi_{L,q}(-\theta_c t|r)\phi_{N,q}(-\theta_c t|r)f_{r,q}(r)dr \bigg] t^{-1}dt \nonumber
   \end{align}
    \normalsize
   (1) is obtained by averaging over the distibution of the serving distance and by using the total law of probability; (2) is obtained by developing the expressions of the conditioned probabilities.
  %%%%%%%%%%%%%%%%%%%%%%%%%%
  
